A 2-category of chronological cobordisms and odd Khovanov homology

We create a framework for odd Khovanov homology in the spirit of Bar-Natan's construction for the ordinary Khovanov homology. Namely, we express the cube of resolutions of a link diagram as a diagram in a certain 2-category of chronological cobordisms and show that it is 2-commutative: the composition of 2-morphisms along any 3-dimensional subcube is trivial. This allows us to create a chain complex, whose homotopy type modulo certain relations is a link invariant. Both the original and the odd Khovanov homology can be recovered from this construction by applying certain strict 2-functors. We describe other possible choices of functors, including the one that covers both homology theories and another generalizing dotted cobordisms to the odd setting. Our construction works as well for tangles and is conjectured to be functorial up to sign with respect to tangle cobordisms.

==> diag-rels.tex <==
\makeatletter

\def\defPictRel#1(#2)(#3)#4{%
	\expandafter\def\csname pictRel#1\endcsname{\@ifstar{%
		\begin{pspicture}(#2)(#3)%
			\psset{linewidth=1pt,dimen=outer,arrowlength=0.8,arrowsize=5pt}%
			#4%
		\end{pspicture}}{%
		\begin{centerpict}(#2)(#3)%
			\psset{linewidth=1pt,dimen=outer,arrowlength=0.8,arrowsize=5pt}%
			#4%
		\end{centerpict}}}%
}

\defPictRel{HoleCreateBirth}(0,-0.5)(2.2,0.5){%
			\pscircle(1.2,0){0.3}
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.22, 0.22)
				\psline( 0.1414,-0.1414)( 0.22,-0.22)
				\psline(-0.1414, 0.1414)(-0.22, 0.22)
				\psline(-0.1414,-0.1414)(-0.22,-0.22)
			}
			\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
			\pscircle[linestyle=dotted,linewidth=0.5pt](0.3,0){0.3}
}

\defPictRel{MergeCreateBirth}(0,-0.5)(2.2,0.5){%
			\pscircle(0.3,0){0.3}
			\pscircle(1.2,0){0.3}
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.22, 0.22)
				\psline( 0.1414,-0.1414)( 0.22,-0.22)
				\psline(-0.1414, 0.1414)(-0.22, 0.22)
				\psline(-0.1414,-0.1414)(-0.22,-0.22)
			}
			\psline[linewidth=2pt]{-}(0.6,0)(0.9,0)
			\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
}

\defPictRel{SplitCreateBirth}(0.6,-0.5)(2.2,0.5){%
			\psclip{\psellipse(1.05,0)(0.45,0.3)}
				\psline[linewidth=2pt]{-}(1.05,-0.3)(1.05,0.3)
			\endpsclip
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.22, 0.22)
				\psline( 0.1414,-0.1414)( 0.22,-0.22)
				\psline(-0.1414, 0.1414)(-0.22, 0.22)
				\psline(-0.1414,-0.1414)(-0.22,-0.22)
			}
			\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
}

\defPictRel{HoleCreateDeath}(0,-0.5)(2.2,0.5){%
			\pscircle(1.2,0){0.3}
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.06, 0.06)
				\psline( 0.1414,-0.1414)( 0.06,-0.06)
				\psline(-0.1414, 0.1414)(-0.06, 0.06)
				\psline(-0.1414,-0.1414)(-0.06,-0.06)
			}
			\psline[linewidth=2pt]{<-}(1.5,0)(1.8,0)
			\pscircle[linestyle=dotted,linewidth=0.5pt](0.3,0){0.3}
}

\defPictRel{MergeCreateDeath}(0,-0.5)(2.2,0.5){%
			\pscircle(0.3,0){0.3}
			\pscircle(1.2,0){0.3}
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.06, 0.06)
				\psline( 0.1414,-0.1414)( 0.06,-0.06)
				\psline(-0.1414, 0.1414)(-0.06, 0.06)
				\psline(-0.1414,-0.1414)(-0.06,-0.06)
			}
			\psline[linewidth=2pt]{<-}(1.5,0)(1.8,0)
			\psline[linewidth=2pt]{-}(0.6,0)(0.9,0)
}

\defPictRel{SplitCreateDeath}(0.6,-0.5)(2.2,0.5){%
			\psclip{\psellipse(1.05,0)(0.45,0.3)}
				\psline[linewidth=2pt]{-}(1.05,-0.3)(1.05,0.3)
			\endpsclip
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.06, 0.06)
				\psline( 0.1414,-0.1414)( 0.06,-0.06)
				\psline(-0.1414, 0.1414)(-0.06, 0.06)
				\psline(-0.1414,-0.1414)(-0.06,-0.06)
			}
			\psline[linewidth=2pt]{<-}(1.5,0)(1.8,0)
}
		
\defPictRel{HHH}(0,-0.6)(3,0.6){%
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(0.3,0){0.3}
			\pscircle(1.5,0){0.3}
			\pscircle(2.7,0){0.3}
}

\defPictRel{HLine}(0,-0.6)(3,0.6){%
			\pscircle(1.2,0){0.25}
			\pscircle(2.8,0){0.25}
			\psellipse(2,0)(0.5,0.3)
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(0.3,0){0.3}
			\pscircle(1.5,0){0.3}
			\pscircle(2.5,0){0.3}
}

\defPictRel{HMesh}(0,-0.6)(3,0.6){%
			\psbezier(1.5,0)(1.1, 0.4)(1, 0.5)(2, 0.5)
			\psbezier(1.5,0)(1.1,-0.4)(1,-0.5)(2,-0.5)
			\psbezier(2.5,0)(2.9, 0.4)(3, 0.5)(2, 0.5)
			\psbezier(2.5,0)(2.9,-0.4)(3,-0.5)(2,-0.5)
			\psellipse(2,0)(0.5,0.3)
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(0.3,0){0.3}
			\pscircle(1.5,0){0.3}
			\pscircle(2.5,0){0.3}
}

\defPictRel{Line}(0,-0.5)(3,0.5){%
			\pscircle(0.2,0){0.25}
			\pscircle(2.8,0){0.25}
			\psellipse(1,0)(0.5,0.3)
			\psellipse(2,0)(0.5,0.3)
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(0.5,0){0.3}
			\pscircle(1.5,0){0.3}
			\pscircle(2.5,0){0.3}
}

\defPictRel{Triangle}(-1,-1)(1,1.2){%
			\pspolygon(-0.52,-0.3)(0.52,-0.3)(0,0.6)
			\pscircle(0,0.9){0.25}
			\pscircle(-0.72,-0.5){0.25}
			\pscircle( 0.72,-0.5){0.25}
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(-0.52,-0.3){0.3}
			\pscircle( 0.52,-0.3){0.3}
			\pscircle( 0.00, 0.6){0.3}
}

\defPictRel{Trefoil}(-1,-1)(1,1.2){%
			\psellipse(0,-0.6)(0.7,0.2)
			\rput{120}(0,0){\psellipse(0,-0.6)(0.7,0.2)}
			\rput{240}(0,0){\psellipse(0,-0.6)(0.7,0.2)}
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(-0.52,-0.3){0.3}
			\pscircle( 0.52,-0.3){0.3}
			\pscircle( 0.00, 0.6){0.3}
}

\defPictRel{VirtBor}(-0.7,-1)(2.3,0.5){%
			\psset{linewidth=1pt,dimen=outer,arrowlength=0.8,arrowsize=5pt}%
			\pscircle(0.3,0.3){1}
			\pscircle(1.3,0.3){1}
			\pscircle(0.8,1.1){1}
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(0.3,0.3){0.3}
			\pscircle(1.3,0.3){0.3}
			\pscircle(0.8,1.1){0.3}
}	

\makeatother

\def\pictRelCreateExplain{
	\psset{linewidth=1pt,dimen=outer,arrowlength=0.8,arrowsize=5pt}%
	\left[\begin{centerpict}(0,-0.3)(2.2,0.3)
		\pscustom{%
			\psarc(0.32,0){0.3}{45}{315}
			\psarcn(0.75,-0.42){0.3}{135}{45}
			\psarc(1.18,0){0.3}{-135}{135}
			\psarcn(0.75,0.42){0.3}{-45}{-135}
		}
		\rput(2,0){\pscircle(0,0){0.2}
			\psline( 0.1414, 0.1414)( 0.22, 0.22)
			\psline( 0.1414,-0.1414)( 0.22,-0.22)
			\psline(-0.1414, 0.1414)(-0.22, 0.22)
			\psline(-0.1414,-0.1414)(-0.22,-0.22)
		}
		\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
	\end{centerpict}\right]\star
	\left[\begin{centerpict}(0,-0.3)(2.2,0.3)
		\pscircle(0.3,0){0.3}
		\pscircle(1.2,0){0.3}
		\rput(2,0){\pscircle(0,0){0.2}
			\psline( 0.1414, 0.1414)( 0.22, 0.22)
			\psline( 0.1414,-0.1414)( 0.22,-0.22)
			\psline(-0.1414, 0.1414)(-0.22, 0.22)
			\psline(-0.1414,-0.1414)(-0.22,-0.22)
		}
		\psline[linewidth=2pt](0.6,0)(0.9,0)
	\end{centerpict}\right]
		=
	\left[\begin{centerpict}(0,-0.3)(2.2,0.3)
		\pscircle(0.3,0){0.3}
		\pscircle(1.2,0){0.3}
		\rput(2,0){\pscircle(0,0){0.2}
			\psline( 0.1414, 0.1414)( 0.22, 0.22)
			\psline( 0.1414,-0.1414)( 0.22,-0.22)
			\psline(-0.1414, 0.1414)(-0.22, 0.22)
			\psline(-0.1414,-0.1414)(-0.22,-0.22)
		}
		\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
	\end{centerpict}\right]\star
	\left[\begin{centerpict}(0,-0.3)(2.4,0.3)
		\pscircle(0.3,0){0.3}
		\pscircle(1.2,0){0.3}
		\pscircle(2.1,0){0.3}
		\psline[linewidth=2pt](0.6,0)(0.9,0)
		\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
	\end{centerpict}\right]^{-1}
}

%%
%%	Diagrams for the proof of Conn = Dis
%%
\def\pictRelDisConn#1#2#3{%
	\ifx\relax#1\relax
		\begin{centerpict}(1.55,-0.5)(3.55,0.5)
	\else\ifx\relax#3\relax
		\begin{centerpict}(0.95,-0.5)(2.95,0.5)
	\else
		\begin{centerpict}(0.95,-0.5)(3.55,0.5)
	\fi\fi
	\ifx1#2\relax
		\pscustom{%
			\moveto(2.95,0)
			\psarc(2.7,0){0.25}{0}{135}
			\psarcn(2.25,0.45){0.386}{-45}{-135}
			\psarc(1.8,0){0.25}{45}{315}
			\psarcn(2.25,-0.45){0.386}{135}{45}
			\psarc(2.7,0){0.25}{-135}{0}
		}
	\else
		\pscircle(1.8,0){0.25}
		\pscircle(2.7,0){0.25}
		\ifx*#2\relax
			\psline[linewidth=3pt,arrowsize=7pt,arrowlength=1]{->}(2.05,0)(2.45,0)
	\fi\fi
	\ifx\relax#1\relax\else
		\pscircle(1.2,0){0.25}
		\pscircle[linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid](1.5,0){0.3}
		\rput(1.5,0){$#1$}
	\fi
	\ifx\relax#3\relax\else
		\pscircle(3.3,0){0.25}
		\pscircle[linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid](3.0,0){0.3}
		\rput(3.0,0){$#3$}
	\fi
	\end{centerpict}
}


==> events-nontransverse.tex <==
\psset{unit=0.4cm}
\begin{pspicture}(0,0)(35,10)
%%
%%	Axes
%%	
\rput(1,3){
	\psline{->}(0,0)(0, 4)\uput[l](0, 4){$f_{t,s}$}
	\psline{->}(0,0)(3,-1)\uput[u](3,-1){$s$}
	\psline{->}(0,0)(2, 2)\uput[u](2, 2){$t$}
}
%%
%%	Creation-annihilation
%%
\rput(6,2){
	% bottom layer
	\psbezier(0,2)(1,3)(1,2)(2,3)\psbezier(2,3)(3,4)(3,5)(4,6)
	% top layer
	\psbezier[border=2\pslinewidth,linewidth=0.3\pslinewidth](2.2,5.2)(5.5,4.1)(5,3.6)(5.9,3.3)
	\psbezier(0,2)(1,3)(1,4)(2,5)\psbezier(2,5)(3,6)(3,5)(4,6)
	\psbezier[linewidth=0.3\pslinewidth](1.8,2.8)(4,2.5)(5,3.6)(5.9,3.3)
	% singular set
	\psbezier[linewidth=0.3\pslinewidth](4,6)(6.1,5.5)(6.9,4.3)(5.9,3.3)
	\psbezier[linewidth=0.3\pslinewidth](0,2)(3,1)(4.9,2.3)(5.9,3.3)
}
%%
%%	Annihilation-creation
%%
\rput(13,0){
	% singular set
	\psbezier[linewidth=0.3\pslinewidth](1.75,4.75)(3.25,4.25)(5,4)(5.5,4.5)
	\psbezier[linewidth=0.3\pslinewidth](3.25,6.25)(4.75,5.75)(6,5)(5.5,4.5)
	% bottom layer
	\psbezier[linewidth=0.3\pslinewidth](5.5,4.5)(6.4,4.2)(7.5,4)(8.5,2.5)
	\psline[linewidth=0.3\pslinewidth](5,7)(11,5)			% back
	\psline[linewidth=0.3\pslinewidth](0,2)(6,0)			%	front
	\psline(6,0)(11,5)													%	right
	\psbezier(0,2)(0.75,3.75)(1,4)(1.75,4.75)		% left
	\psbezier(5,7)(4.25,7.00)(4,7)(3.25,6.25)		% left
	% top layer
	\psline[border=2\pslinewidth](6,2)(11,7)															% right
	\psline[border=2\pslinewidth,linewidth=0.3\pslinewidth](0,4)(6,2)			%	front
	\psline[linewidth=0.3\pslinewidth](5,9)(11,7)													% back
	\psbezier(0,4)(0.75,4.00)(1,4)(1.75,4.75)				% left
	\psbezier(5,9)(4.25,7.25)(4,7)(3.25,6.25)				% left
	\psbezier[linewidth=0.3\pslinewidth](5.5,4.5)(6.4,4.2)(7.5,4)(8.5,4.5)
}
%%
%%	Permutations
%%
\rput(24,0){
	% singular set
	\psbezier[linewidth=0.3\pslinewidth](1.09136,4.09136)(4.09136,3.09136)(5.25,4.25)(5.5,4.5)
	\psbezier[linewidth=0.3\pslinewidth](3.90864,6.90864)(6.90864,5.90864)(5.75,4.75)(5.5,4.5)
	% bottom layer
	\psbezier(5,9)(4,7.5)(3.5,5.5)(2.5,4.5)		% left right-top
	\psline[linewidth=0.3\pslinewidth](5,7)(11,5)			% back
	\psline[linewidth=0.3\pslinewidth](0,2)(6,0)			%	front
	\psline(6,0)(11,5)													%	right
	% mimina-maxima line
	\psbezier[border=2\pslinewidth,linewidth=0.3\pslinewidth](2.5,6.5)(3.6,6)(5,5.5)(5.5,4.5)
	\psbezier(0,2)(1,3.5)(1.5,5.5)(2.5,6.5)		% left left-bottom
	% mimina-maxima lines
	\psbezier[linewidth=0.3\pslinewidth](5.5,4.5)(6,3.5)(7.4,3)(8.5,2.5)
	\psbezier[linewidth=0.3\pslinewidth](2.5,4.5)(3.6,4)(5,4.2)(5.5,4.5)
	% top layer
	\psline[border=2\pslinewidth](6,2)(11,7)															% right
	\psline[border=2\pslinewidth,linewidth=0.3\pslinewidth](0,4)(6,2)			%	front
	\psline[linewidth=0.3\pslinewidth](5,9)(11,7)													% back
	\psbezier(5,7)(4,6.5)(3.5,7.5)(2.5,6.5)		% left right-bottom
	\psbezier(0,4)(1,4.5)(1.5,3.5)(2.5,4.5)		% left left-top
	% mimina-maxima line
	\psbezier[linewidth=0.3\pslinewidth](5.5,4.5)(6,4.8)(7.4,5)(8.5,4.5)
}
\end{pspicture}

%
% 2-3.5-5.5-6.5
% 4-4.5-3.5-4.5
%
% 2,2,-2,-2


==> events-two.tex <==
\psset{unit=0.4cm}
\begin{pspicture}(0,0)(35,10)
%%
%%	Axes
%%	
\rput(1,4){
	\psline{->}(0,0)(0, 4)\uput[l](0, 4){$f_{t,s}$}
	\psline{->}(0,0)(3,-1)\uput[u](3,-1){$s$}
	\psline{->}(0,0)(2, 2)\uput[u](2, 2){$t$}
}
%%
%%	Switching two permutations
%%
\rput(8,0){
	% bottom layer
	\psline[linewidth=0.3\pslinewidth](5, 7)(11,5)											%	back bottom
	\psline[border=2\pslinewidth](8,3)(11,6)\psbezier(6,0)(7,1)(7,2)(8,3)	% right bottom -> top
	\psline[linewidth=0.3\pslinewidth](5, 8)(11,6)											% back top
	\psline(0,2)(3,5)\psbezier(3,5)(4,6)(4,7)(5,8)			% left bottom -> top
	\psline[linewidth=0.3\pslinewidth](0,2)(6,0)												% front bottom
	\psline[border=2\pslinewidth,linewidth=0.3\pslinewidth](0,3)(6,1)		% front top
	\psline(0,3)(3,6)\psbezier(3,6)(4,7)(4,6)(5,7)			% left top -> bottom
	\psline(8,2)(11,5)\psbezier(6,1)(7,2)(7,1)(8,2)			% right top -> bottom
	\psline[linewidth=0.3\pslinewidth](4,6.5)(7,1.5)		% singular line
	% top layer
	\psline[linewidth=5\pslinewidth,linecolor=white](1,5.5)(10,6.5)		% singular line shadow
	\psline[linewidth=5\pslinewidth,linecolor=white](0,4)(6,2)				% front bottom shadow
	\psline[linewidth=5\pslinewidth,linecolor=white](0,5)(6,3)				% front top shadow
	\psline[linewidth=0.3\pslinewidth](5, 9)(11,7)			% back bottom
	\psline[border=2\pslinewidth](6,2)(9,5)\psbezier[border=2\pslinewidth](9,5)(10,6)(10,7)(11,8)		% right bottom -> top
	\psline(2,7)(5,10)\psbezier(0,4)(1,5)(1,6)(2,7)		% left bottom -> top
	\psline[border=2\pslinewidth,linewidth=0.3\pslinewidth](0,5)(6,3)			% front top
	\psline(2,6)(5, 9)\psbezier(0,5)(1,6)(1,5)(2,6)		% left top -> bottom
	\psline[border=2\pslinewidth](6,3)(9,6)\psbezier(9,6)(10,7)(10,6)(11,7)		% right top -> bottom
	\psline[linewidth=0.3\pslinewidth](5,10)(11,8)		% back top
	\psline[linewidth=0.3\pslinewidth](0,4)(6,2)			% front bottom
	\psline[linewidth=0.3\pslinewidth](1,5.5)(10,6.5)		% singular line
}
%%
%%	Switching a creation with a permutation
%%
\rput(22,0){
	% bottom layer
	\psline[linewidth=0.3\pslinewidth](5, 7)(11,5)											%	back bottom
	\psline[border=2\pslinewidth](8,3)(11,6)\psbezier(6,0)(7,1)(7,2)(8,3)	% right bottom -> top
	\psline[linewidth=0.3\pslinewidth](5, 8)(11,6)											% back top
	\psline(0,2)(3,5)\psbezier(3,5)(4,6)(4,7)(5,8)			% left bottom -> top
	\psline[linewidth=0.3\pslinewidth](0,2)(6,0)												% front bottom
	\psline[border=2\pslinewidth,linewidth=0.3\pslinewidth](0,3)(6,1)		% front top
	\psline(0,3)(3,6)\psbezier(3,6)(4,7)(4,6)(5,7)			% left top -> bottom
	\psline(8,2)(11,5)\psbezier(6,1)(7,2)(7,1)(8,2)			% right top -> bottom
	\psline[linewidth=0.3\pslinewidth](4,6.5)(7,1.5)		% singular line
	% top layer
	\psline[border=2\pslinewidth,linewidth=0.3\pslinewidth](1,5.5)(8.5,5)		% singular line: top
	\psbezier[linecolor=white,linewidth=5\pslinewidth](8.5,5)(9.5,6)(10,6)(11,7)		% right bottom (white)
	\psline[linewidth=0.3\pslinewidth](5, 9)(11,7)						% back bottom
	\psbezier[border=2\pslinewidth](8.5,5)(9.5,6)(10,7)(11,8)		% right top
	\psbezier(8.5,5)(9.5,6)(10,6)(11,7)													% right bottom
	\psline[linewidth=0.3\pslinewidth](5,10)(11,8)						% back top
	\psbezier(1,5.5)(2,6.5)(2,7)(5,10)		%	left top
	\psbezier(1,5.5)(2,6.5)(2,6)(5, 9)		% left bottom
}
\end{pspicture}


==> images/diag-rels.tex <==
\makeatletter

\def\defPictRel#1(#2)(#3)#4{%
	\expandafter\def\csname pictRel#1\endcsname{\@ifstar{%
		\begin{pspicture}(#2)(#3)%
			\psset{linewidth=1pt,dimen=outer,arrowlength=0.8,arrowsize=5pt}%
			#4%
		\end{pspicture}}{%
		\begin{centerpict}(#2)(#3)%
			\psset{linewidth=1pt,dimen=outer,arrowlength=0.8,arrowsize=5pt}%
			#4%
		\end{centerpict}}}%
}

\defPictRel{HoleCreateBirth}(0,-0.5)(2.2,0.5){%
			\pscircle(1.2,0){0.3}
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.22, 0.22)
				\psline( 0.1414,-0.1414)( 0.22,-0.22)
				\psline(-0.1414, 0.1414)(-0.22, 0.22)
				\psline(-0.1414,-0.1414)(-0.22,-0.22)
			}
			\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
			\pscircle[linestyle=dotted,linewidth=0.5pt](0.3,0){0.3}
}

\defPictRel{MergeCreateBirth}(0,-0.5)(2.2,0.5){%
			\pscircle(0.3,0){0.3}
			\pscircle(1.2,0){0.3}
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.22, 0.22)
				\psline( 0.1414,-0.1414)( 0.22,-0.22)
				\psline(-0.1414, 0.1414)(-0.22, 0.22)
				\psline(-0.1414,-0.1414)(-0.22,-0.22)
			}
			\psline[linewidth=2pt]{-}(0.6,0)(0.9,0)
			\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
}

\defPictRel{SplitCreateBirth}(0.6,-0.5)(2.2,0.5){%
			\psclip{\psellipse(1.05,0)(0.45,0.3)}
				\psline[linewidth=2pt]{-}(1.05,-0.3)(1.05,0.3)
			\endpsclip
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.22, 0.22)
				\psline( 0.1414,-0.1414)( 0.22,-0.22)
				\psline(-0.1414, 0.1414)(-0.22, 0.22)
				\psline(-0.1414,-0.1414)(-0.22,-0.22)
			}
			\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
}

\defPictRel{HoleCreateDeath}(0,-0.5)(2.2,0.5){%
			\pscircle(1.2,0){0.3}
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.06, 0.06)
				\psline( 0.1414,-0.1414)( 0.06,-0.06)
				\psline(-0.1414, 0.1414)(-0.06, 0.06)
				\psline(-0.1414,-0.1414)(-0.06,-0.06)
			}
			\psline[linewidth=2pt]{<-}(1.5,0)(1.8,0)
			\pscircle[linestyle=dotted,linewidth=0.5pt](0.3,0){0.3}
}

\defPictRel{MergeCreateDeath}(0,-0.5)(2.2,0.5){%
			\pscircle(0.3,0){0.3}
			\pscircle(1.2,0){0.3}
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.06, 0.06)
				\psline( 0.1414,-0.1414)( 0.06,-0.06)
				\psline(-0.1414, 0.1414)(-0.06, 0.06)
				\psline(-0.1414,-0.1414)(-0.06,-0.06)
			}
			\psline[linewidth=2pt]{<-}(1.5,0)(1.8,0)
			\psline[linewidth=2pt]{-}(0.6,0)(0.9,0)
}

\defPictRel{SplitCreateDeath}(0.6,-0.5)(2.2,0.5){%
			\psclip{\psellipse(1.05,0)(0.45,0.3)}
				\psline[linewidth=2pt]{-}(1.05,-0.3)(1.05,0.3)
			\endpsclip
			\rput(2,0){\pscircle(0,0){0.2}
				\psline( 0.1414, 0.1414)( 0.06, 0.06)
				\psline( 0.1414,-0.1414)( 0.06,-0.06)
				\psline(-0.1414, 0.1414)(-0.06, 0.06)
				\psline(-0.1414,-0.1414)(-0.06,-0.06)
			}
			\psline[linewidth=2pt]{<-}(1.5,0)(1.8,0)
}
		
\defPictRel{HHH}(0,-0.6)(3,0.6){%
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(0.3,0){0.3}
			\pscircle(1.5,0){0.3}
			\pscircle(2.7,0){0.3}
}

\defPictRel{HLine}(0,-0.6)(3,0.6){%
			\pscircle(1.2,0){0.25}
			\pscircle(2.8,0){0.25}
			\psellipse(2,0)(0.5,0.3)
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(0.3,0){0.3}
			\pscircle(1.5,0){0.3}
			\pscircle(2.5,0){0.3}
}

\defPictRel{HMesh}(0,-0.6)(3,0.6){%
			\psbezier(1.5,0)(1.1, 0.4)(1, 0.5)(2, 0.5)
			\psbezier(1.5,0)(1.1,-0.4)(1,-0.5)(2,-0.5)
			\psbezier(2.5,0)(2.9, 0.4)(3, 0.5)(2, 0.5)
			\psbezier(2.5,0)(2.9,-0.4)(3,-0.5)(2,-0.5)
			\psellipse(2,0)(0.5,0.3)
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(0.3,0){0.3}
			\pscircle(1.5,0){0.3}
			\pscircle(2.5,0){0.3}
}

\defPictRel{Line}(0,-0.5)(3,0.5){%
			\pscircle(0.2,0){0.25}
			\pscircle(2.8,0){0.25}
			\psellipse(1,0)(0.5,0.3)
			\psellipse(2,0)(0.5,0.3)
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(0.5,0){0.3}
			\pscircle(1.5,0){0.3}
			\pscircle(2.5,0){0.3}
}

\defPictRel{Triangle}(-1,-1)(1,1.2){%
			\pspolygon(-0.52,-0.3)(0.52,-0.3)(0,0.6)
			\pscircle(0,0.9){0.25}
			\pscircle(-0.72,-0.5){0.25}
			\pscircle( 0.72,-0.5){0.25}
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(-0.52,-0.3){0.3}
			\pscircle( 0.52,-0.3){0.3}
			\pscircle( 0.00, 0.6){0.3}
}

\defPictRel{Trefoil}(-1,-1)(1,1.2){%
			\psellipse(0,-0.6)(0.7,0.2)
			\rput{120}(0,0){\psellipse(0,-0.6)(0.7,0.2)}
			\rput{240}(0,0){\psellipse(0,-0.6)(0.7,0.2)}
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(-0.52,-0.3){0.3}
			\pscircle( 0.52,-0.3){0.3}
			\pscircle( 0.00, 0.6){0.3}
}

\defPictRel{VirtBor}(-0.7,-1)(2.3,0.5){%
			\psset{linewidth=1pt,dimen=outer,arrowlength=0.8,arrowsize=5pt}%
			\pscircle(0.3,0.3){1}
			\pscircle(1.3,0.3){1}
			\pscircle(0.8,1.1){1}
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(0.3,0.3){0.3}
			\pscircle(1.3,0.3){0.3}
			\pscircle(0.8,1.1){0.3}
}	

\makeatother

\def\pictRelCreateExplain{
	\psset{linewidth=1pt,dimen=outer,arrowlength=0.8,arrowsize=5pt}%
	\left[\begin{centerpict}(0,-0.3)(2.2,0.3)
		\pscustom{%
			\psarc(0.32,0){0.3}{45}{315}
			\psarcn(0.75,-0.42){0.3}{135}{45}
			\psarc(1.18,0){0.3}{-135}{135}
			\psarcn(0.75,0.42){0.3}{-45}{-135}
		}
		\rput(2,0){\pscircle(0,0){0.2}
			\psline( 0.1414, 0.1414)( 0.22, 0.22)
			\psline( 0.1414,-0.1414)( 0.22,-0.22)
			\psline(-0.1414, 0.1414)(-0.22, 0.22)
			\psline(-0.1414,-0.1414)(-0.22,-0.22)
		}
		\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
	\end{centerpict}\right]\star
	\left[\begin{centerpict}(0,-0.3)(2.2,0.3)
		\pscircle(0.3,0){0.3}
		\pscircle(1.2,0){0.3}
		\rput(2,0){\pscircle(0,0){0.2}
			\psline( 0.1414, 0.1414)( 0.22, 0.22)
			\psline( 0.1414,-0.1414)( 0.22,-0.22)
			\psline(-0.1414, 0.1414)(-0.22, 0.22)
			\psline(-0.1414,-0.1414)(-0.22,-0.22)
		}
		\psline[linewidth=2pt](0.6,0)(0.9,0)
	\end{centerpict}\right]
		=
	\left[\begin{centerpict}(0,-0.3)(2.2,0.3)
		\pscircle(0.3,0){0.3}
		\pscircle(1.2,0){0.3}
		\rput(2,0){\pscircle(0,0){0.2}
			\psline( 0.1414, 0.1414)( 0.22, 0.22)
			\psline( 0.1414,-0.1414)( 0.22,-0.22)
			\psline(-0.1414, 0.1414)(-0.22, 0.22)
			\psline(-0.1414,-0.1414)(-0.22,-0.22)
		}
		\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
	\end{centerpict}\right]\star
	\left[\begin{centerpict}(0,-0.3)(2.4,0.3)
		\pscircle(0.3,0){0.3}
		\pscircle(1.2,0){0.3}
		\pscircle(2.1,0){0.3}
		\psline[linewidth=2pt](0.6,0)(0.9,0)
		\psline[linewidth=2pt]{->}(1.5,0)(1.8,0)
	\end{centerpict}\right]^{-1}
}

%%
%%	Diagrams for the proof of Conn = Dis
%%
\def\pictRelDisConn#1#2#3{%
	\ifx\relax#1\relax
		\begin{centerpict}(1.55,-0.5)(3.55,0.5)
	\else\ifx\relax#3\relax
		\begin{centerpict}(0.95,-0.5)(2.95,0.5)
	\else
		\begin{centerpict}(0.95,-0.5)(3.55,0.5)
	\fi\fi
	\ifx1#2\relax
		\pscustom{%
			\moveto(2.95,0)
			\psarc(2.7,0){0.25}{0}{135}
			\psarcn(2.25,0.45){0.386}{-45}{-135}
			\psarc(1.8,0){0.25}{45}{315}
			\psarcn(2.25,-0.45){0.386}{135}{45}
			\psarc(2.7,0){0.25}{-135}{0}
		}
	\else
		\pscircle(1.8,0){0.25}
		\pscircle(2.7,0){0.25}
		\ifx*#2\relax
			\psline[linewidth=3pt,arrowsize=7pt,arrowlength=1]{->}(2.05,0)(2.45,0)
	\fi\fi
	\ifx\relax#1\relax\else
		\pscircle(1.2,0){0.25}
		\pscircle[linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid](1.5,0){0.3}
		\rput(1.5,0){$#1$}
	\fi
	\ifx\relax#3\relax\else
		\pscircle(3.3,0){0.25}
		\pscircle[linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid](3.0,0){0.3}
		\rput(3.0,0){$#3$}
	\fi
	\end{centerpict}
}

==> images/pics-tangles.tex <==
\newlength\fntinkwidth
\newlength\fntsize
\newlength\fntshift
\newbox\fntbox

\makeatletter

%% \defPicFonts{family}{name}(x0,y0)(x1,y1):size:<size_factor>[r|c|<empty>|outline_code]{code}

\def\defPicFonts#1#2{\@ifnextchar(%
	{\defPicFonts@getcoords{#1}{#2}}%
	{\defPicFonts@getsize{#1}{#2}(-0.5,-0.5)(0.5,0.5)}}
	
\def\defPicFonts@getcoords#1#2(#3){\@ifnextchar(%
	{\defPicFonts@getsize{#1}{#2}(#3)}%
	{\defPicFonts@getsize{#1}{#2}(0,0)(#3)}}

\def\defPicFonts@getsize#1#2(#3)(#4){\@ifnextchar:%)
	{\defPicFonts@getsizefactor{#1}{#2}{(#3)(#4)}}%
	{\defPicFonts@getsizefactor{#1}{#2}{(#3)(#4)}:W:}}
	
\def\defPicFonts@getsizefactor#1#2#3:#4:{\@ifnextchar<%>
	{\defPicFonts@getoutline{#1}{#2}{#3}{#4}}%
	{\defPicFonts@getoutline{#1}{#2}{#3}{#4}<1>}}

\def\defPicFonts@getoutline#1#2#3#4<#5>{\@ifnextchar[%]
	{\defPicFonts@getcode{#1}{#2}{#3}{#4}{#5}}%
	{\defPicFonts@getcode{#1}{#2}{#3}{#4}{#5}[]}}

\def\defPicFonts@getcode#1#2#3#4#5[#6]#7{%
	\ifx#6r\relax
		\defPicFonts@define{#1}{#2}{#3}{#4}{#5}{\psframe[linewidth=0.3pt,linestyle=dotted]#3}{#7}%
	\else\ifx#6c\relax
		\defPicFonts@define{#1}{#2}{#3}{#4}{#5}{\pscircle[linewidth=0.3pt,linestyle=dotted](0,0){0.5}}{#7}%
	\else
		\defPicFonts@define{#1}{#2}{#3}{#4}{#5}{#6}{#7}%
	\fi\fi
}

%% \defPicFonts@define{family}{name}{coords}{hbox_for_size}{size_factor}{outline_code}{code}
%%
\def\defPicFonts@define#1#2#3#4#5#6#7{%
	%
	%	#1#2 draws the symbol using PS-Tricks unit
	% starred version: with outline
	\expandafter\edef\csname#1#2\endcsname{%
		\noexpand\@ifstar
			{\expandafter\noexpand\csname#1#2@draw\endcsname\noexpand\iftrue\noexpand\fi}%
			{\expandafter\noexpand\csname#1#2@draw\endcsname\noexpand\iffalse\noexpand\fi}}%
	%
	% The drawing macro; ##1 = (\iffalse|\iftrue) and ##2 = \fi determine the presence of the outline
	\expandafter\def\csname#1#2@draw\endcsname##1##2{\begingroup
		\pspicture#3%
			\psset{linewidth=0.5pt,dotsep=1pt,arrowsize=5pt,arrowlength=1}%
			##1#6##2#7%
		\endpspicture\endgroup}%
	%
	% fnt#1#2 draws the symbol as a font
	% starred version: no outline
	\expandafter\edef\csname fnt#2\endcsname{%
		\noexpand\@ifstar
			{\expandafter\noexpand\csname fnt#2@size\endcsname\noexpand\iftrue\noexpand\fi}%
			{\expandafter\noexpand\csname fnt#2@size\endcsname\noexpand\iffalse\noexpand\fi}}%
	%
	% The drawing macro; ##1 = (\iffalse|\iftrue) and ##2 = \fi determine the presence of the outline
	\expandafter\def\csname fnt#2@size\endcsname##1##2{%
		\def\fnt@drawcode{#7##1#6##2}%
		\ifmmode
			\edef\next{\noexpand\mathchoice
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\textfont\noexpand\displaystyle}%
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\textfont\noexpand\textstyle}%
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\scriptfont\noexpand\scriptstyle}%
				{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\scriptscriptfont\noexpand\scriptscriptstyle}}%
		\else
			\edef\next{\expandafter\noexpand\csname fnt#2@draw\endcsname\noexpand\textfont\noexpand\textstyle}%
		\fi
		\next
	}
	\expandafter\def\csname fnt#2@draw\endcsname##1##2{\begingroup
		\fntinkwidth=\fontdimen8##13\relax
		\setbox\fntbox=\hbox{$\m@th##2#4$}%
		\fntshift= \dp\fntbox	\fntshift=#5\fntshift
		\fntsize = \ht\fntbox	\fntsize=#5\fntsize	\advance\fntsize\fntshift
		\psset{unit=\fntsize,linewidth=\fntinkwidth,dotsep=1pt,arrowsize=7\pslinewidth,arrowlength=0.8,arrowinset=0.6}%
		\hskip\fntinkwidth\ifmmode
			\vcenter{\hbox{\pspicture#3\fnt@drawcode\endpspicture}}%
		\else
			\pspicture[shift=-\fntshift]#3\fnt@drawcode\endpspicture
		\fi\hskip\fntinkwidth
	\endgroup}
}

\makeatother

%%
%%	Crossings and resolutions
%%
\defPicFonts{big}{Circle}:|:{\pscircle[linewidth=0.5pt](0,0.05){0.45}}

\defPicFonts{big}{NWSECr}[r]{%
		\psline(-0.5,-0.5)(0.5,0.5)
		\psline[border=3\pslinewidth](-0.5,0.5)(0.5,-0.5)
}%

\defPicFonts{big}{NESWCr}[r]{%
		\psline(-0.5,0.5)(0.5,-0.5)
		\psline[border=3\pslinewidth](-0.5,-0.5)(0.5,0.5)
}%

\defPicFonts{big}{VertRes}[r]{%
		\psbezier(-0.5,-0.5)(-0.08,0)(-0.08,0)(-0.5,0.5)
		\psbezier( 0.5,-0.5)( 0.08,0)( 0.08,0)( 0.5,0.5)
}%

\defPicFonts{big}{HorRes}[r]{%
		\psbezier(-0.5,-0.5)(0,-0.08)(0,-0.08)(0.5,-0.5)
		\psbezier(-0.5, 0.5)(0, 0.08)(0, 0.08)(0.5, 0.5)
}%

\defPicFonts{big}{HorResCob}[r]{%
		\psbezier(-0.5,-0.5)(0,-0.08)(0,-0.08)(0.5,-0.5)
		\psbezier(-0.5, 0.5)(0, 0.08)(0, 0.08)(0.5, 0.5)
		\psline[linewidth=3\pslinewidth](0,-0.18)(0,0.18)
}%

\defPicFonts{big}{PosCr}[r]{%
		\psline{->}(0.5,-0.5)(-0.55,0.55)
		\psline[border=3\pslinewidth]{->}(-0.5,-0.5)(0.55,0.55)
}%

\defPicFonts{big}{NegCr}[r]{%
		\psline{->}(-0.5,-0.5)(0.55,0.55)
		\psline[border=3\pslinewidth]{->}(0.5,-0.5)(-0.55,0.55)
}%

\defPicFonts{big}{NoCr}[r]{%
		\psbezier{->}(-0.5,-0.5)(-0.08,0)(-0.08,0)(-0.55,0.55)
		\psbezier{->}( 0.5,-0.5)( 0.08,0)( 0.08,0)( 0.55,0.55)
}%

\defPicFonts{big}{PosCrArrowUp}[r]{%
		\psline(0.5,-0.5)(-0.55,0.55)
		\psline[border=5\pslinewidth](-0.5,-0.5)(0.55,0.55)
		\psline[linewidth=0.5\pslinewidth,border=1\pslinewidth]{->}(0,-0.5)(0,0.7)
}%

\defPicFonts{big}{PosCrArrowDown}[r]{%
		\psline(0.5,-0.5)(-0.55,0.55)
		\psline[border=5\pslinewidth](-0.5,-0.5)(0.55,0.55)
		\psline[linewidth=0.5\pslinewidth,border=1\pslinewidth]{<-}(0,-0.7)(0,0.5)
}%

%%
%%	A horizontal full twist tangle
%%
\defPicFonts{tangle}{FullTwist}:|:<1.25>[c]{%
	\psclip{\psframe[linestyle=none](0,-1)(1,1)}
		\psbezier(-0.433, 0.25)(-0.15,-0.33)(0.15,-0.33)(0.433, 0.25)
	\endpsclip
	\psbezier[border=3\pslinewidth](-0.433,-0.25)(-0.15, 0.33)(0.15, 0.33)(0.433,-0.25)
	\psclip{\psframe[linestyle=none](0.1,-1)(-1,1)}
		\psbezier[border=3\pslinewidth](-0.433, 0.25)(-0.15,-0.33)(0.15,-0.33)(0.433, 0.25)
	\endpsclip
}

%%
%%	Twisted unknots
%%
\defPicFonts{tangle}{PosTwist}(-1,-0.5)(1,0.5)[r]{%
	\psbezier{C-C}( 0.5,-0.5)( 0.2,-0.5)(-0.2,0.5)(-0.5,0.5)
	\psbezier[border=3\pslinewidth]{C-C}(-0.5,-0.5)(-0.2,-0.5)( 0.2,0.5)( 0.5,0.5)
	\psarc{C-C}(-0.5,0){0.5}{90}{270}%
	\psarc{C-C}(0.5,0){0.5}{-90}{90}%
}

\defPicFonts{tangle}{PosTwistHor}(-1,-0.5)(1,0.5)[r]{\pscustom{%
	\moveto(-0.5,0.5)
	\psarc(-0.5,0){0.5}{90}{270}\curveto(-0.3,-0.5)(-0.2,-0.2)(0,-0.2)\curveto( 0.2,-0.2)( 0.3,-0.5)( 0.5,-0.5)
	\psarc( 0.5,0){0.5}{-90}{90}\curveto( 0.3, 0.5)( 0.2, 0.2)(0, 0.2)\curveto(-0.2, 0.2)(-0.3, 0.5)(-0.5, 0.5)
	\stroke
}}

\defPicFonts{tangle}{PosTwistVert}(-1,-0.5)(1,0.5)[r]{%
	\psarc{C-C}( 0.5,0){0.5}{-90}{90}\psellipticarc{C-C}( 0.5,0)(0.4,0.5){90}{270}%
	\psarc{C-C}(-0.5,0){0.5}{90}{270}\psellipticarc{C-C}(-0.5,0)(0.4,0.5){-90}{90}%
}

%%
%%	First Reidemeister move
%%
\defPicFonts{tangle}{RIline}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.25355, 0.15355)(0, 0.2)(0,0)
	\psbezier(-0.35355,-0.35355)(-0.25355,-0.15355)(0,-0.2)(0,0)
}

\defPicFonts{tangle}{RIx}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.25355, 0.15355)(-0.1,-0.2)(0.1,-0.2)
	\psbezier[border=3\pslinewidth](-0.35355,-0.35355)(-0.25355,-0.15355)(-0.1, 0.2)(0.1, 0.2)
	\psbezier(0.1,0.2)(0.4,0.2)(0.4,-0.2)(0.1,-0.2)
}
	
\defPicFonts{tangle}{RIh}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.2, 0)(-0.1, 0.2)(0.1, 0.2)
	\psbezier(0.1,0.2)(0.4,0.2)(0.4,-0.2)(0.1,-0.2)
	\psbezier(-0.35355,-0.35355)(-0.2, 0)(-0.1,-0.2)(0.1,-0.2)
}

\defPicFonts{tangle}{RIv}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.2,0)(-0.2,0)(-0.35355,-0.35355)
	\pscircle(0.1,0){0.2}
}

\defPicFonts{tangle}{RIcob}:|:<1.25>[c]{%
	\psbezier(-0.35355, 0.35355)(-0.2,0)(-0.2,0)(-0.35355,-0.35355)
	\pscircle(0.1,0){0.2}
	\psline[linewidth=3\pslinewidth](-0.24,0)(-0.1,0)
}

%%
%%	Second Reidemeister move
%%
\defPicFonts{tangle}{RIIxx}:|:<1.25>[c]{%
	\psbezier(-0.433, 0.25)(-0.15,-0.33)(0.15,-0.33)(0.433, 0.25)
	\psbezier[border=3\pslinewidth](-0.433,-0.25)(-0.15, 0.33)(0.15, 0.33)(0.433,-0.25)
}

\defPicFonts{tangle}{RIIhh}:|:<1.25>[c]{%
	\psbezier(-0.433, 0.25)(-0.3,-0.1)(-0.2, 0.2)(0, 0.2)
	\psbezier(-0.433,-0.25)(-0.3, 0.1)(-0.2,-0.2)(0,-0.2)
	\psbezier(0.433, 0.25)(0.3,-0.1)(0.2, 0.2)(0, 0.2)
	\psbezier(0.433,-0.25)(0.3, 0.1)(0.2,-0.2)(0,-0.2)
}

\defPicFonts{tangle}{RIIhv}:|:<1.25>[c]{%
	\psbezier(0.433,0.25)(0.3,0)(0.3,0)(0.433,-0.25)
	\psarc(0,0){0.2}{-90}{90}
	\psbezier(-0.433, 0.25)(-0.3,-0.1)(-0.2, 0.2)(0, 0.2)
	\psbezier(-0.433,-0.25)(-0.3, 0.1)(-0.2,-0.2)(0,-0.2)
}

\defPicFonts{tangle}{RIIvh}:|:<1.25>[c]{%
	\psbezier(-0.433,0.25)(-0.3,0)(-0.3,0)(-0.433,-0.25)
	\psarc(0,0){0.2}{90}{270}
	\psbezier(0.433, 0.25)(0.3,-0.1)(0.2, 0.2)(0, 0.2)
	\psbezier(0.433,-0.25)(0.3, 0.1)(0.2,-0.2)(0,-0.2)
}

\defPicFonts{tangle}{RIIvv}:|:<1.25>[c]{%
	\psbezier(-0.433,0.25)(-0.3,0)(-0.3,0)(-0.433,-0.25)
	\pscircle(0,0){0.2}
	\psbezier(0.433,0.25)(0.3,0)(0.3,0)(0.433,-0.25)
}

\defPicFonts{tangle}{RIIhhs}:|:<1.25>[c]{%
	\psbezier(-0.433, 0.25)(-0.2,0)(0.2,0)(0.433, 0.25)
	\psbezier(-0.433,-0.25)(-0.2,0)(0.2,0)(0.433,-0.25)
}

%%
%%	Third Reidemeister move
%%
\defPicFonts{tangle}{RIIIax}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(0.35355,0.35355)
	\psline[border=2\pslinewidth](-0.35355,0.35355)(0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIah}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIav}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)(-0.35355, 0.35355)
	\psbezier( 0.35355, 0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIac}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psline[linewidth=5\pslinewidth](0,-0.08839)(0,0.08839)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,0.35)(0,0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,0.35)(0,0.35)
}

\defPicFonts{tangle}{RIIIahhh}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
	\psarc(0,0.2){0.15}{45}{315}
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIahhv}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\pscircle(0,0.2){0.15}
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
	\psbezier( 0.35355, 0.35355)( 0.2,0.2)( 0.25,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIahvh}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\psarc(0,0.2){0.15}{45}{135}
	\psarc(0,0.2){0.15}{225}{315}
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIahvv}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0.05, 0.05)(-0.05, 0.05)( 0.35355,-0.35355)
	\psbezier( 0.35355, 0.35355)(0.2,0.2)(0.25,0)(0.5,0)
	\psarc(0,0.2){0.15}{-135}{135}
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
}

\defPicFonts{tangle}{RIIIavhh}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{45}{225}
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
}

\defPicFonts{tangle}{RIIIavhv}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{-45}{225}
	\psbezier(-0.35355, 0.35355)(-0.2,0.2)(-0.25,0)(-0.5,0)
	\psbezier( 0.35355, 0.35355)( 0.2,0.2)( 0.25,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIavvh}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{45}{135}
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
	\psbezier(0.10607,0.30607)(0.15607,0.25607)(0.2,0.2)(0.35355,0.35355)
	\psbezier(0.10607,0.09393)(0.25607,0.24393)(0.3,0)( 0.5,0)
}

\defPicFonts{tangle}{RIIIavvv}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(-0.10607,-0.10607)
	\psline( 0.35355,-0.35355)( 0.10607,-0.10607)
	\psarc(-0.20607,-0.00607){0.14142}{-45}{45}
	\psarc( 0.20607,-0.00607){0.14142}{135}{225}
	\psarc(0,0.2){0.15}{-45}{135}
	\psbezier( 0.35355, 0.35355)(0.2,0.2)(0.25,0)(0.5,0)
	\psbezier(-0.10607,0.30607)(-0.15607,0.25607)(-0.2,0.2)(-0.35355,0.35355)
	\psbezier(-0.10607,0.09393)(-0.25607,0.24393)(-0.3,0)(-0.5,0)
}

\defPicFonts{tangle}{RIIIbx}:|:<1.25>[c]{%
	\psline(-0.35355,-0.35355)(0.35355,0.35355)
	\psline[border=2\pslinewidth](-0.35355,0.35355)(0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

\defPicFonts{tangle}{RIIIbh}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

\defPicFonts{tangle}{RIIIbv}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)(-0.35355, 0.35355)
	\psbezier( 0.35355, 0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

\defPicFonts{tangle}{RIIIbc}:|:<1.25>[c]{%
	\psbezier(-0.35355,-0.35355)(0,0)(0,0)( 0.35355,-0.35355)
	\psbezier(-0.35355, 0.35355)(0,0)(0,0)( 0.35355, 0.35355)
	\psline[linewidth=5\pslinewidth](0,-0.08839)(0,0.08839)
	\psbezier[border=2\pslinewidth](-0.5,0)(-0.25,0)(-0.2,-0.35)(0,-0.35)
	\psbezier[border=2\pslinewidth]( 0.5,0)( 0.25,0)( 0.2,-0.35)(0,-0.35)
}

%%
%%	Three horizontal lines
%%
\defPicFonts{tangle}{IIIVert}:|:<1.25>[c]{%
	\psbezier(-0.35355,0.35355)(-0.08,0.08)(0.08,0.08)(0.35355,0.35355)
	\psline(-0.5,0)(0.5,0)
	\psbezier(-0.35355,-0.35355)(-0.08,-0.08)(0.08,-0.08)(0.35355,-0.35355)
}

\defPicFonts{tangle}{IIIVertT}:|:<1.25>[c]{%
	\psbezier(-0.35355,0.35355)(-0.08,0.08)(0.08,0.08)(0.35355,0.35355)
	\psline(-0.5,0)(0.5,0)
	\psbezier(-0.35355,-0.35355)(-0.08,-0.08)(0.08,-0.08)(0.35355,-0.35355)
	\psline[linewidth=3\pslinewidth](0,0)(0,0.14839)
}

\defPicFonts{tangle}{IIIVertB}:|:<1.25>[c]{%
	\psbezier(-0.35355,0.35355)(-0.08,0.08)(0.08,0.08)(0.35355,0.35355)
	\psline(-0.5,0)(0.5,0)
	\psbezier(-0.35355,-0.35355)(-0.08,-0.08)(0.08,-0.08)(0.35355,-0.35355)
	\psline[linewidth=3\pslinewidth](0,0)(0,-0.14839)
}

%%
%%	Passing a circle over a link
%%
\defPicFonts{tangle}{CircLeft}(-0.375,-0.5)(0.5,0.5):|:<1.25>[r]{%
	\psline(0.375,-0.5)(0.375,0.5)
	\pscircle(0,0){0.25}
}
\defPicFonts{tangle}{CircRight}(-0.5,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\psline(-0.375,-0.5)(-0.375,0.5)
	\pscircle(0,0){0.25}
}
\defPicFonts{tangle}{CircOver}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\psline(0,-0.5)(0,0.5)
	\pscircle[border=3\pslinewidth](0,0){0.25}
}
\defPicFonts{tangle}{CircUnder}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\pscircle(0,0){0.25}
	\psline[border=3\pslinewidth](0,-0.5)(0,0.5)
}

\defPicFonts{tangle}{CircOverhh}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\pscustom{\moveto(0,-0.5)
		\curveto(0,-0.125)(0.25,-0.3)(0.25,0)
		\curveto(0.25,0.15)(0,0.35)(0,0)
		\curveto(0,-0.35)(-0.25,-0.15)(-0.25,0)
		\curveto(-0.25,0.3)(0,0.125)(0,0.5)
		\stroke
	}
}
\defPicFonts{tangle}{CircOverhv}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\pscustom{\moveto(0,-0.5)\curveto(0,-0.125)(0.25,-0.3)(0.25,0)\curveto(0.25,0.3)(0,0.125)(0,0.5)\stroke}%
	\pscustom{\moveto(0,0)\curveto(0,-0.35)(-0.25,-0.15)(-0.25,0)\curveto(-0.25,0.15)(0,0.35)(0,0)\stroke}%
}
\defPicFonts{tangle}{CircOvervh}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\pscustom{\moveto(0,-0.5)\curveto(0,-0.125)(-0.25,-0.3)(-0.25,0)\curveto(-0.25,0.3)(0,0.125)(0,0.5)\stroke}%
	\pscustom{\moveto(0,0)\curveto(0,-0.35)(0.25,-0.15)(0.25,0)\curveto(0.25,0.15)(0,0.35)(0,0)\stroke}%
}
\defPicFonts{tangle}{CircOvervv}(-0.375,-0.5)(0.375,0.5):|:<1.25>[r]{%
	\pscustom{\moveto(0,-0.5)
		\curveto(0,-0.125)(-0.25,-0.3)(-0.25,0)
		\curveto(-0.25,0.15)(0,0.35)(0,0)
		\curveto(0,-0.35)(0.25,-0.15)(0.25,0)
		\curveto(0.25,0.3)(0,0.125)(0,0.5)
		\stroke
	}
}


==> khovanov-pict.tex <==
\begingroup
\def\cobordism{%
	\rput(0,0){\psclip{\pscustom[linestyle=none]{%
			\moveto(-1.40851, 0.73936)
			\lineto(-0.97994, 0.73936)
			\lineto(-0.97994, 0.00325)
			\lineto( 0.41979,-0.52933)
			\curveto(0.41979, 0.47067)( 0.72783, 0.58117)(0.72783,-0.41883)
			\lineto( 1.66534,-0.49630)
			\lineto( 1.66534, 1)
			\lineto(-1.40851, 1)}}
		\psset{linestyle=dashed,dash=1pt 1.5pt,linewidth=0.15pt}
		\psbezier(-1.2,0.84)(-0.6,0.84)( 0.43607,0.19574)( 0.65569,-0.168)
		\psbezier(-1.2,0.84)(-1.8,0.84)(-0.99532,0.19574)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)(-1.25766,-0.05626)(-1.08,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.41841,-0.05626)( 0.12,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.85886,-0.78374)(0.64393,-0.53174)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)( 0.38039,-0.78374)(0.87532,-0.53174)( 0.65569,-0.168)
		\psset{linestyle=none,fillcolor=white,fillstyle=solid}
		\psellipse(0.48,-0.462)(0.35,0.35)
		\psellipse(0.24, 0.231)(0.25,0.25)
		\psellipse(-0.9, 0.231)(0.25,0.25)
		\psset{linestyle=dashed,fillstyle=none}
		\psbezier(0.03970,0.37025)(0.12403,0.31650)(0.09682,0.26530)(-0.00150,0.28352)
		\psbezier(0.43596,0.07651)(0.36107,0.14277)(0.39169,0.19477)( 0.48781,0.16718)
		\psbezier(-0.97994,0.00325)(-1.01341,0.09748)(-0.78568,0.15397)(-0.69968,0.10295)
		\psbezier(-0.67676,0.31978)(-0.77519,0.30210)(-1.01856,0.30893)(-1.09755,0.37025)
		\psbezier(0.15998,-0.30309)(0.34781,-0.37181)(0.64296,-0.64475)(0.14597,-0.58989)
		\psbezier(0.82952,-0.50660)(0.63507,-0.45979)(0.81076,-0.42482)(0.65569,-0.168)
	\endpsclip}
	\rput(0,0){\psclip{\pscustom[linestyle=none]{%
			\moveto(-1.40851, 0.73936)
			\lineto(-0.97994, 0.73936)
			\lineto(-0.97994, 0.00325)
			\lineto( 0.41979,-0.52933)
			\curveto(0.41979, 0.47067)( 0.72783, 0.58117)(0.72783,-0.41883)
			\lineto( 1.66534,-0.49630)
			\lineto( 1.8,-0.49630)
			\lineto( 1.8,-1)
			\lineto(-1.6,-1)
			\lineto(-1.6, 0.73936)}}
		\psset{linestyle=solid,linewidth=0.5pt}
		\psbezier(-1.2,0.84)(-0.6,0.84)( 0.43607,0.19574)( 0.65569,-0.168)
		\psbezier(-1.2,0.84)(-1.8,0.84)(-0.99532,0.19574)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)(-1.25766,-0.05626)(-1.08,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.41841,-0.05626)( 0.12,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.85886,-0.78374)(0.64393,-0.53174)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)( 0.38039,-0.78374)(0.87532,-0.53174)( 0.65569,-0.168)
		\psset{linestyle=none,fillcolor=white,fillstyle=solid}
		\psellipse(0.48,-0.462)(0.35,0.32)
		\psellipse(0.24, 0.231)(0.25,0.25)
		\psellipse(-0.9, 0.231)(0.25,0.25)
		\psset{linestyle=solid,fillstyle=none}
		\psbezier(0.03970,0.37025)(0.12403,0.31650)(0.09682,0.26530)(-0.00150,0.28352)
		\psbezier(0.43596,0.07651)(0.36107,0.14277)(0.39169,0.19477)( 0.48781,0.16718)
		\psbezier(-0.97994,0.00325)(-1.01341,0.09748)(-0.78568,0.15397)(-0.69968,0.10295)
		\psbezier(-0.67676,0.31978)(-0.77519,0.30210)(-1.01856,0.30893)(-1.09755,0.37025)
		\psbezier(0.15998,-0.30309)(0.34781,-0.37181)(0.64296,-0.64475)(0.14597,-0.58989)
		\psbezier(0.82952,-0.50660)(0.63507,-0.45979)(0.81076,-0.42482)(0.65569,-0.168)
	\endpsclip}
	\rput(0,1.5){%
		\psset{linestyle=solid,linewidth=0.5pt}
		\psbezier(-1.2,0.84)(-0.6,0.84)( 0.43607,0.19574)( 0.65569,-0.168)
		\psbezier(-1.2,0.84)(-1.8,0.84)(-0.99532,0.19574)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)(-1.25766,-0.05626)(-1.08,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.41841,-0.05626)( 0.12,0.336)(-0.48,0.336)
		\psbezier( 1.63924,-0.42)( 1.85886,-0.78374)(0.64393,-0.53174)(-0.17569,-0.168)
		\psbezier(-0.43924,-0.42)( 0.38039,-0.78374)(0.87532,-0.53174)( 0.65569,-0.168)
		\psset{linestyle=none,fillcolor=white,fillstyle=solid}
		\psellipse(0.48,-0.462)(0.35,0.32)
		\psellipse(0.24, 0.231)(0.25,0.25)
		\psellipse(-0.9, 0.231)(0.25,0.25)
		\psset{linestyle=solid,fillstyle=none}
		\psbezier(0.03970,0.37025)(0.12403,0.31650)(0.09682,0.26530)(-0.00150,0.28352)
		\psbezier(0.43596,0.07651)(0.36107,0.14277)(0.39169,0.19477)( 0.48781,0.16718)
		\psbezier(-0.97994,0.00325)(-1.01341,0.09748)(-0.78568,0.15397)(-0.69968,0.10295)
		\psbezier(-0.67676,0.31978)(-0.77519,0.30210)(-1.01856,0.30893)(-1.09755,0.37025)
		\psbezier(0.15998,-0.30309)(0.34781,-0.37181)(0.81076,-0.42482)(0.65569,-0.168)
		\psbezier(0.82952,-0.50660)(0.63507,-0.45979)(0.44416,-0.62280)(0.14597,-0.58989)
	}
	\rput(0,0){%
		\psset{linewidth=0.5pt,dash=1pt 1.5pt}
		\psline{c-c}(-1.40851, 0.73936)(-1.40851,2.25000)
		\psline{c-c}(-0.97994, 0.00325)(-0.97994,1.50325)
		\psdash\psline{c-c}( 0.08996, 0.31025)( 0.08996,1.221)
		\psdash\psline{c-c}( 0.39409, 0.14265)( 0.39409,1.14265)
		\psline{-c}( 0.08996, 1.221)( 0.08996,1.81025)
		\psline{-c}( 0.39409, 1.14265)( 0.39409,1.64265)
		\psline{c-c}( 1.66534,-0.49630)( 1.66534,1.00370)
		\psbezier{c-c}( 0.41979,-0.52933)( 0.41979,0.47067)( 0.72783, 0.58117)(0.72783,-0.41883)
		\rput(0.58652,0.2782){\psline[linewidth=0.3pt,arrowsize=4pt,arrowlength=1]{->}(0.1,0.1)(-0.4,-0.05)}
	}
}

\def\cubevertex#1#2#3{\begingroup
	\psset{linewidth=0.8pt,linestyle=solid}%
	\begin{pspicture}(-1,-0.8)(1,1.1)%
		\pspolygon[fillcolor=white,fillstyle=solid,linestyle=none](-1,-0.8)(1,-0.8)(1,1.2)(-1,1.2)
		\trefoilresolution{#1}{#2}{#3}%
		\rput*[t](0,-0.85){\small $#1#2#3$}%
	\end{pspicture}%
\endgroup}

\def\cubeedge#1#2#3{\begingroup
	\psset{linewidth=0.5pt,linestyle=solid,unit=0.5}%
	\begin{centerpict}(-0.8,-0.7)(0.8,1)%
		\trefoilresolution{#1}{#2}{#3}%
	\end{centerpict}%
\endgroup}

\begin{pspicture}(0,0)(16.5,13)
%	\pspolygon[linewidth=1pt,linestyle=dotted,linecolor=blue](0,0)(16.5,0)(16.5,13)(0,13)
	% Top left corner: knot diagram
	\rput[tl](0,13){$\left\llbracket\trefoil aca\right\rrbracket$}
	% Bottom: chain complex
	\rput( 2.1, 0.5){\Rnode[href=-0.25]{C0}{\Large $C^0$}}
	\rput( 6.4, 0.5){\Rnode[href=-0.25]{C1}{\Large $C^1$}}
	\rput(10.7, 0.5){\Rnode[href=-0.25]{C2}{\Large $C^2$}}
	\rput(15.0, 0.5){\Rnode[href=-0.25]{C3}{\Large $C^3$}}
	\begingroup
	\psset{linestyle=solid,linewidth=1pt,nodesep=3pt,arrowsize=4.5pt}
	\ncline{->}{C0}{C1}	\naput{$d$}
	\ncline{->}{C1}{C2}	\naput{$d$}
	\ncline{->}{C2}{C3}	\naput{$d$}
	\endgroup
	% Vertical dotted lines --- direct sum
	\pnode( 2.0, 8){col0}
	\pnode( 6.3,12){col1}
	\pnode(10.6,12){col2}
	\pnode(14.9, 8){col3}
	\begingroup
	\psset{linestyle=dotted,linewidth=1pt,nodesep=3pt,arrowsize=5pt}
	\ncline{->}{col0}{C0}
	\ncline{->}{col1}{C1}	\uput[r]( 6.3,1.7){$\cdot\,\{1\}$}
	\ncline{->}{col2}{C2}	\uput[r](10.6,1.7){$\cdot\,\{2\}$}
	\ncline{->}{col3}{C3}	\uput[r](14.9,1.7){$\cdot\,\{3\}$}
	\endgroup
	% Resolutions
	\rput( 2.0, 8){\rnode{000}{\cubevertex{0}{0}{0}}}
	\rput( 6.3,12){\rnode{100}{\cubevertex{1}{0}{0}}}
	\rput( 6.3, 8){\rnode{010}{\cubevertex{0}{1}{0}}}
	\rput( 6.3, 4){\rnode{001}{\cubevertex{0}{0}{1}}}
	\rput(10.6,12){\rnode{110}{\cubevertex{1}{1}{0}}}
	\rput(10.6, 8){\rnode{101}{\cubevertex{1}{0}{1}}}
	\rput(10.6, 4){\rnode{011}{\cubevertex{0}{1}{1}}}
	\rput(14.9, 8){\rnode{111}{\cubevertex{1}{1}{1}}}
	\begingroup
	\psset{linestyle=solid,linewidth=1pt,nodesep=-2pt,labelsep=1pt,arrowsize=5pt}
	\ncline{->}{000}{100}		\nbput{$\scriptstyle {*}00$}	\naput{\cubeedge{a}{0}{0}}
	\ncline{->}{000}{010}		\nbput{$\scriptstyle 0{*}0$}	\naput{\cubeedge{0}{c}{0}}
	\ncline{->}{000}{001}		\nbput{$\scriptstyle 00{*}$}	\naput{\cubeedge{0}{0}{a}}
	\ncline{->}{010}{110}	\nbput[npos=0.15]{$\scriptstyle {*}10$}
												\naput[npos=0.12]{$-\permMM$\cubeedge{a}{1}{0}}
	\ncline{->}{010}{011}	\naput[npos=0.20]{$\scriptstyle 01{*}$}
												\naput[npos=0.85]{$\!\!\!\!\!\!\!-\permMM$\cubeedge{0}{1}{a}}
	\ncline{->}{100}{110}	\nbput[npos=0.50]{$\scriptstyle 1{*}0$}
												\naput{\cubeedge{1}{c}{0}}
	\ncline[border=2pt]{->}{100}{101}	\naput[npos=0.20]{$\scriptstyle 10{*}$}
																		\naput[npos=0.80]{\cubeedge{1}{0}{a}}
	\ncline[border=2pt]{->}{001}{101}	\nbput[npos=0.15]{$\scriptstyle {*}01$}
																		\naput[npos=0.15]{$-\permMM$\cubeedge{a}{0}{1}}
	\ncline{->}{001}{011}	\naput{$\scriptstyle 0{*}1$}
												\nbput{\cubeedge{0}{c}{1}}
	\ncline{->}{110}{111}	\nbput[npos=0.5]{$\scriptstyle 11{*}$}
												\naput{\cubeedge{1}{1}{a}}
	\ncline{->}{101}{111}	\nbput[npos=0.5]{$\scriptstyle 1{*}1$}
												\naput[npos=0.35]{$-\permMM$\cubeedge{1}{c}{1}}
	\ncline{->}{011}{111}	\naput[npos=0.5]{$\scriptstyle {*}11$}
												\nbput{$\!\!\!\!-\permSS$\cubeedge{a}{1}{1}}
	\endgroup
	%% cobordism
	\rput(1.5,3){\begingroup
		\psframe[linestyle=none,fillstyle=solid,fillcolor=white](0.3,-0.6)(0.7,1.5)
		\psset{yunit=0.64,xunit=0.8}
		\cobordism
	\endgroup}
	\pscurve[border=1pt,linewidth=0.3pt,arrowsize=4pt]{->}(4.15,7.5)(4,7)(3,6)(2.7,5.5)(2.2,4.3)
\end{pspicture}
\endgroup


==> linearization-old.tex <==
\subsection*{Linearization}
%%
%%	Linearization
%%
The~$2$-category $\ChCob(0)$ is not good for homological constructions and we will
\quot{linearize} it. More precisely, choose a~commutative ring $R$ and assume
there is a~function $\iota\colon 2\Mor(\ChCob(0))\to R$ that is multiplicative with
respect to both compositions of $2$-morphisms. Define a~$2$-category $R\ChCob_\iota(0)$
as follows:
\begin{enumerate}
	\item the~set of objects is not changed and it consists of families of circles in $\Disk$,
	\item morphisms are finite linear combinations of chronological cobordisms
				\begin{displaymath}
					r_1W_1 + \ldots + r_kW_k
				\end{displaymath}
				with $r_i\in R$, modulo \emph{chronological relations} $W'=\iota(\varphi)W$, one
				for each $2$-morphism $\varphi\colon W\to W'$ in $\ChCob(0)$, and
	\item $2$-morphisms are elements of $R$ acting by a~multiplication, i.e. there is
				a~$2$-morphism $r\colon W\Rightarrow W'$ whenever $r\cdot W = W'$.
\end{enumerate}
We extend the~composition of cobordisms to formal sums in a~linear way. Both vertical and
horizontal compositions of $2$-morphisms are given by multiplication in $R$. A~function $\iota$
mentioned above induces a~monoidal $2$-functor $\iota\colon\ChCob(0)\to R\ChCob_/\iota(0)$,
which we denote by the~same letter. We want it to be rich enough to support the~construction
of odd Khovanov homology. We start with a~few observations.

%%
%%	Annihilation and creation are equalities
%%
\begin{lemma}
	We can assume $\iota$ maps creations and annihilations into equalities.
\end{lemma}
\begin{proof}
	Each of the~three creations \eqref{change:creation-annihilation} involves different
	generators. Hence, we can force the~coefficients associated to them to be $1$ by
	scaling a~birth and deaths.
\end{proof}

%%
%%	Disjoint permutations -  only degrees matter
%%
\begin{lemma}\label{lem:coeff-disjoint-degree}
	The~coefficient $\iota_W^{W'} := \iota\!\left(\sigma_{W,W'}\colon W\ldsum W'\Rightarrow W\rdsum W'\right)$
	associated to a~disjoint permutation depends only on degrees of $W$ and $W'$. In particular, there
	is a~function
	\begin{equation}\label{eq:lambda-function}
		\lambda\colon\Z\times\Z\to R, \qquad (a,b,c,d) \mapsto \permMM^{ac}\permSS^{bd}\permMS^{ad-bc},
	\end{equation}
	such that $\iota_W^{W'} = \lambda(\deg W, \deg W')$. The~coefficients $\permMM,\permSS,\permMS\in R$
	are some invertible elements and $\permMM^2=\permSS^2=1$.
\end{lemma}
\begin{proof}
	If such a~function exists, then both $\permMM$ and $\permSS$ squared must be equal to $1$,
	because the~inverse of $\sigma_{W,W}$ is given by itself conjugated with a~twist. To see that
	$\iota_W^{W'}$ depends only on degrees of $W$ and $W'$, it is enough to show that permutations
	of any cobordism with a~merge and with a~birth have inverse coefficients --- this follows
	immediately from triviality of the~following change of a~chronology:
	\begin{equation}\label{eq:rel-create-perm}
						\psset{unit=0.8}
						\begin{centerpict}(-0.2,0)(1.6,2.4)
							\cobordism[1](0,0)(I)(I)
							\cobordism[1](1.2,0)(I)(I)
							\psframe[fillstyle=solid,fillcolor=white](-0.2,0.7)(1.4,1.7)
							\rput(0.8,0.2){$\scriptstyle\cdots$}
							\rput(0.8,2.2){$\scriptstyle\cdots$}
							\rput(0.6,1.2){$W$}
						\end{centerpict}
						\Longrightarrow
						\begin{centerpict}(-0.2,0)(2.4,2.9)
							\cobordism[1](0,0)(sI)(I)(I)
							\cobordism[1](1.2,0)(I)(srB,2)(rM-R)
							\psframe[fillstyle=solid,fillcolor=white](-0.2,0.3)(1.4,1.3)
							\rput(0.8,0.1){$\scriptstyle\cdots$}
							\rput(0.8,2.2){$\scriptstyle\cdots$}
							\rput(0.6,0.8){$W$}
						\end{centerpict}
						\Longrightarrow
						\begin{centerpict}(-0.2,0)(2.4,2.9)
							\cobordism[1](0,0)(sI)(I)(I)
							\cobordism[1](1.2,0)(srB,2)(rM-R)(I)
							\psframe[fillstyle=solid,fillcolor=white](-0.2,1.6)(1.4,2.6)
							\rput(0.8,0.7){$\scriptstyle\cdots$}
							\rput(0.8,2.8){$\scriptstyle\cdots$}
							\rput(0.6,2.1){$W$}
						\end{centerpict}
						\Longrightarrow
						\begin{centerpict}(-0.2,0)(1.6,2.4)
							\cobordism[1](0,0)(I)(I)
							\cobordism[1](1.2,0)(I)(I)
							\psframe[fillstyle=solid,fillcolor=white](-0.2,0.7)(1.4,1.7)
							\rput(0.8,0.2){$\scriptstyle\cdots$}
							\rput(0.8,2.2){$\scriptstyle\cdots$}
							\rput(0.6,1.2){$W$}
						\end{centerpict}
	\end{equation}
	where $W$ is any cobordism. The~same holds for a~split and any death.
\end{proof}

The~above implies the~following table of coefficients for disjoint permutations
$\sigma_{W,W'}$ between cobordisms with a~single critical point.
\begin{center}
	\def\arraystretch{1.5}
	\begin{tabular}{c|cccc}
		\begin{centerpict}(0,0)(1,1)
			\rput[bl](-0.05,0.15){$W$}
			\rput[tr](1.05,0.85){$W'$}
			\psline[linewidth=0.3pt](0.2,0.8)(0.8,0.2)
		\end{centerpict}
		& birth & merge & split & death \\
		\hline
		birth & $\permMM$ & $\permMM$ & $\permSM$ & $\permMS$ \\
		merge & $\permMM$ & $\permMM$ & $\permMS$ & $\permSM$ \\
		split & $\permMS$ & $\permSM$ & $\permSS$ & $\permSS$ \\
		death & $\permSM$ & $\permMS$ & $\permSS$ & $\permSS$
	\end{tabular}
\end{center}
For instance, we have the~following equalities
\begin{equation}
	\psset{unit=0.8cm}
	\permMM\textcobordism[2](M-L)(sI)\textcobordism[0](I)(sB)
	\ =
	\ \textcobordism[2](sI)(M-L)\hskip\COBxsize\psxunit\textcobordism[0](sB)(I)
	\qquad\textrm{and}\qquad
	\permMS\textcobordism[2](M-L)(sI)\textcobordism[1](sI)(S-B)
	\ =
	\textcobordism[2](sI)(M-L)\hskip\COBxsize\psxunit\textcobordism[1](S-B)(sI)\,.
\end{equation}
It remains to define $\iota$ for the~remaining permutation changes encoded with diagrams
\eqref{change:connected-permutations}. We use the~coefficients from Tab.~\ref{tab:cube-faces}
on page \pageref{tab:cube-faces}.

%%
%%	Definition of \iota
%%
\begin{proposition}
	Choose invertible elements $\permMM,\permSS,\permMS\in R$ such that $\permMM^2=\permSS^2=1$
	and define $\iota$ on generating changes of chronologies by the~following rules:
	\begin{enumerate}
		\item creations and annihilations are sent to equalities,
		\item a~$\times$-change is sent into $\permSS$, if the~arrows point to the~same circle,
					and into $\permMM$ otherwise,
		\item a~$\Diamond$-change with a~diagram in which the~inner arrow is oriented upwards is sent
					into $1$ or $\permMM\permSS$ if the~outer arrow is oriented to the~left or to the~right
					respectively, and
		\item the~coefficient associated to any other change permuting two critical points of degrees
					$(a,b)$ and $(c,d)$ is given by $\lambda(a,b,c,d)=\permMM^{ac}\permSS^{bd}\permMS^{ad-bc}$.
	\end{enumerate}
	Then $\iota\colon\ChCob(0)\to R\ChCob_\iota(0)$ is a~well-defined $2$-functor.
\end{proposition}
\begin{proof}
	We have to check that $\iota$ defined as above is consistent with relations between
	elementary changes of chronologies. These are described by codimension $2$ singularities
	and can be gathered into four groups:
	\begin{enumerate}
		\item changes supported on different regions commute \eqref{rel:far-away},
		\item a~change followed by its inverse is trivial \eqref{rel:inverses},
		\item coherence relations between permutations and creations or annihilations
					\eqref{rel:permutations}, the~top row, and
		\item the~two ways of reversing an~order of three critical points describe
					the~same change of a~chronology \eqref{rel:permutations}, the~bottom row.
	\end{enumerate}
	Coherence of $\iota$ with the~first group of relations follows from the~commutativity of $R$,
	whereas relations from the~second group holds because $\lambda(a,b,c,d)\lambda(c,d,a,b)=1$
	and the~coefficients assigned to $\times$- and $\Diamond$-changes are square roots of $1$.
	The~third group of relations is satisfied due to Lemma~\ref{lem:coeff-disjoint-degree}. Each
	relation from the~last group is an~equality between two changes, each modeled by a~locally
	vertical diffeotopy with respect to three tubes around critical points $a$, $b$ and $c$ in
	a~cobordism $W$. Therefore, we have to check that $\iota$ preserves commutativity of hexagons
	\begin{equation}\label{eq:hexagon-relation}
		\setlength\arraycolsep{5mm}
		\def\arraystretch{2}
		\begin{array}{cccc}
				&  \Rnode[href=-0.5]{bac}{W\raisebox{0.2ex}{$\scriptstyle(b<a<c)$}}
				&  \Rnode[href= 0.5]{bca}{W\raisebox{0.2ex}{$\scriptstyle(b<c<a)$}}
				\\ \Rnode[href= 0.7]{abc}{W\raisebox{0.2ex}{$\scriptstyle(a<b<c)$}} &&
				&  \Rnode[href=-0.7]{cba}{W\raisebox{0.2ex}{$\scriptstyle(c<b<a)$}} \\
				&  \Rnode[href=-0.5]{acb}{W\raisebox{0.2ex}{$\scriptstyle(a<c<b)$}}
				&  \Rnode[href= 0.5]{cab}{W\raisebox{0.2ex}{$\scriptstyle(c<a<b)$}}
		\end{array}
		\begin{diagps}(0,0)(0,0)
			\ncLine{->}{abc}{bac}
			\ncLine{->}{bac}{bca}
			\ncLine{->}{bca}{cba}
			\ncLine{->}{abc}{acb}
			\ncLine{->}{acb}{cab}
			\ncLine{->}{cab}{cba}
		\end{diagps}
	\end{equation}
	where $W\raisebox{0.2ex}{$\scriptstyle(b<a<c)$}$ is a~cobordism obtained from $W$ by placing
	its critical points in the~specified order and each arrow represents an~elementary permutation
	change.
	
	If $W$ is disjoint, say $a$ is in a~component $W_1$ and $b,c$ in a~component $W_2$,
	it is  enough to notice that both $W_2\raisebox{0.2ex}{$\scriptstyle(b<c)$}$ and
	$W_2\raisebox{0.2ex}{$\scriptstyle(c<b)$}$ have the~same degree --- permutating $W_1$
	with both of them results in the~same coefficient.
	
	If $W$ is connected, then all critical points have index $1$. Take a~look at the~singular
	level containing all of them. The~choice for $\iota$ we made satisfies
	\begin{equation}
		\psset{linewidth=0.5pt}
		\iota\!\left(\begin{centerpict}(1,-0.5)(3.5,0.5)
			\pscircle(1.2,0){0.25}
			\pscircle(1.8,0){0.25}
			\pscircle(2.7,0){0.25}
			\pscircle(3.3,0){0.25}
			\psset{linestyle=dotted,fillcolor=white,fillstyle=solid}
			\pscircle(1.5,0){0.3}
			\pscircle(3.0,0){0.3}
			\rput(1.5,0){$A$}
			\rput(3.0,0){$B$}
		\end{centerpict}\right)
		=
		\iota\!\left(\begin{centerpict}(1,-0.5)(3,0.5)
			\pscircle(1.2,0){0.25}
			\pscircle(2.8,0){0.25}
			\psellipse(2,0)(0.5,0.3)
			\psset{linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid}
			\pscircle(1.5,0){0.3}
			\pscircle(2.5,0){0.3}
			\rput(1.5,0){$A$}
			\rput(2.5,0){$B$}
		\end{centerpict}\right)
	\end{equation}
	for any way we insert saddles into holes $A$ and $B$, so that the~following modification
	of the~cobordism $W$
	\begin{center}
		\begin{centerpict}(0,-0.5)(1.8,0.5)
			\pscircle(0.3,0){0.25}
			\psarc(0.9,0){0.25}{90}{270}
			\psline(0.9, 0.25)(1.8, 0.25)
			\psline(0.9,-0.25)(1.8,-0.25)
			\pscircle[linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid](0.6,0){0.3}
		\end{centerpict}
		\quad$\longrightarrow$\quad
		\begin{centerpict}(0,-0.5)(1.8,0.5)
			\pscircle(0.3,0){0.25}
			\pscircle(0.9,0){0.25}
			\psarc(1.8,0){0.25}{90}{270}
			\pscircle[linestyle=dotted,linewidth=0.5pt,fillcolor=white,fillstyle=solid](0.6,0){0.3}
		\end{centerpict}
	\end{center}
	does not affect values of $\iota$ for the~two changes being related. It remains to check
	four more cases listed in Tab.~\ref{tab:chcob3-hexagon-rels}. The~numbers below each
	diagram indicate how many times a~particular elementary change occurs when we go around
	the~hexagon \eqref{eq:hexagon-relation}. In each case, the~product of values of $\iota$
	is equal to $1$.
\end{proof}

\begin{table}
	\psset{linewidth=0.5pt,fillstyle=solid,fillcolor=white}
	\begin{tabular}{cccc}%
		\begin{pspicture}(-1.25,-0.2)(1.25,1)%		A triangle of circles
			\pspolygon[linewidth=1.5pt](-0.519,-0.3)(0.519,-0.3)(0,0.6)
			\pscircle(-0.519,-0.3){0.3}
			\pscircle( 0.519,-0.3){0.3}
			\pscircle(0,0.6){0.3}
		\end{pspicture}&%
		\begin{pspicture}(-1.25,-0.5)(1.25,0.6)%		Two circles, three arrows: one inside and two outside
			\psellipse[linewidth=1.5pt](0,0)(0.8,0.2)
			\pscircle(0.5,0){0.3}
			\psclip{\pscircle(-0.5,0){0.3}}
				\psline[linewidth=1.5pt](-0.8,0)(-0.2,0)
			\endpsclip
		\end{pspicture}&%
		\begin{pspicture}(-1.25,-0.5)(1.25,0.6)%		One circle, two vertical arrows inside, one horizontal outside
			\psellipse[linewidth=1.5pt](0,0.2)(0.7,0.3)
			\psclip{\psellipse(0,0)(0.5,0.3)}
				\psline[linewidth=1.5pt](-0.2,-0.3)(-0.2,0.3)
				\psline[linewidth=1.5pt]( 0.2,-0.3)( 0.2,0.3)
			\endpsclip
		\end{pspicture}&%
		\begin{pspicture}(-1.25,-0.4)(1.25,0.6)%		Two circles with three parallel arrows
			\psline[linewidth=1.5pt](-0.5,-0.3)(0.5,-0.3)
			\psline[linewidth=1.5pt](-0.5, 0  )(0.5, 0  )
			\psline[linewidth=1.5pt](-0.5, 0.3)(0.5, 0.3)
			\psellipse(-0.5,0)(0.3,0.5)
			\psellipse( 0.5,0)(0.3,0.5)
		\end{pspicture}\\
		$\begin{array}{c}\\
									   \scriptstyle(03|00|300)\\
										 \scriptstyle(21|00|300)\end{array}$ &
		$\begin{array}{c}\scriptstyle(10|11|100)\\
										 \scriptstyle(01|20|100)\\
										 \scriptstyle(01|02|100)\end{array}$ &
		$\begin{array}{c}\scriptstyle(10|20|010)\\
										 \scriptstyle(10|02|010)\\
										 \scriptstyle(01|11|010)\end{array}$ &
		$\begin{array}{c}\\
		                 \scriptstyle(30|00|030)\\
										 \scriptstyle(11|00|030)\end{array}$
	\end{tabular}
	\vskip 0.5\baselineskip
	\caption{Singular levels of homotopies relating permutation changes. Numbers below each
	diagram indicate how many times various permutations occur: $\times$-changes with
	parallel or opposite arrows (the~first group), $\Diamond$-changes with outer arrows
	oriented to the~left or to the~right (the~second group) and the~other changes grouped
	by the~value of $\iota$ (respectively $\permMM$, $\permSS$ and $\permMS$). Different
	sequences correspond to different orientations of saddle points.}
	\label{tab:chcob3-hexagon-rels}
\end{table}

\begin{remark}
	We will usually omit the~subscript, writing $R\ChCob(0)$ for the~linearized category.
	If the~choice of $\iota$ is important, we will write $R\ChCob_{abc}(0)$ for the~quotient
	by chronological relations with parameters $\permMM$, $\permSS$ and $\permMS$ set to $a$,
	$b$ and $c$ accordingly.
\end{remark}

%%
%%	Reversing an orientation
%%
\begin{corollary}\label{cor:orientation-rev}
	The~following rules for reversing orientations hold:
	\begin{equation}
		\psset{unit=8mm}%
		\textcobordism[2](M-R) = \permMM\textcobordism[2](M-L),\hskip 1cm
		\textcobordism[1](S-F) = \permSS\textcobordism[1](S-B),\hskip 1cm
		\psset{unit=1cm}%
		\textcobordism[1](sD-) = \permSS\textcobordism[1](sD+).
	\end{equation}
\end{corollary}
\begin{proof}
	The~last rule follows from the~following change
	\begin{equation}\label{eq:reverse-death}
	\textcobordism*[1](I)(sI)(sD+)
		\,\Longrightarrow\,
	\textcobordism*[1](S-B)(slD-)(sD+)
		\,\Longrightarrow\,
	\textcobordism*[1](S-B)(srD+,2)(sD-)
		\,\Longrightarrow\,
	\textcobordism*[1](I)(sI)(sD-)
	\end{equation}
	and the~first one from
	\begin{equation}\label{eq:reverse-merge}
	\psset{unit=8mm}%
	\textcobordism*[2](sI)(M-L)(sI)
		\,\Longrightarrow\,
	\textcobordism*{\COBshortCylinderVert(0,0)\COBshortLeftBirth[1](1.6,0)}
								 {\COBmergeFrRight[3](0,0.6)}
								 {\COBmergeFrLeft(0.4,1.8)}
		\,\Longrightarrow\,
	\textcobordism*{\COBshortCylinderVert(0,0)\COBshortLeftBirth[1](1.6,0)}
								 {\COBmergeFrLeft[3,2](0,0.6)}
								 {\COBmergeFrRight(0.4,1.8)}
		\,\Longrightarrow\,
	\textcobordism*[2](sI)(M-R)(sI)
	\end{equation}
	Reversing an~orientation of a~split is done in a~similar way.
\end{proof}

As explained in Remark~\ref{rmk:many-2-mors}, even if the~space of admissible diffeotopies is
simply connected, there are $2$-automorphisms of chronological cobordisms that are not trivial.
In the~case of $R\ChCob(0)$ there are cobordisms that are annihilated by $1-\permMM\permSS$:
a~disjoint sum of two spheres (permute the~components) and a~twice punctured torus (reverse
orientations of both saddle points and rotate the~cobordism). In fact nothing else can happen.

\begin{theorem}\label{thm:aut(W)}
	Let $R=\Z[\permMM,\permSS,\permMS^{\pm1}]/(\permMM^2=\permSS^2=1)$ and choose an~embedded
	chronological cobordism $W$ in $R\ChCob(0)$. Then
	\begin{equation}
		\Aut(W)=\begin{cases}
						\{1\},&\textrm{if $g(W)=0$ and $W$ has at most one spherical component},\\
						\{1, \permMM\permSS\},&\textrm{otherwise}.\\
					\end{cases}
	\end{equation}
\end{theorem}

\noindent
A~proof of this result uses a~chronological version of Frobenius algebras and is postponed
to Section~\ref{sec:chron-Frob}.
a~chronological version of Frobenius algebras.

